Mobility as an Alternative Communication Channel: A Survey

We review the research literature investigating systems in which mobile entities can carry data while they move. These entities can be either mobile by nature (e.g., human beings and animals) or mobile by design (e.g., trains, airplanes, and cars). The movements of such entities equipped with storage capabilities create a communication channel which can help overcome the limitations or the lack of conventional data networks. Common limitations include the mismatch between the capacity offered by these networks and the traffic demand or their limited deployment owing to environmental factors. Application scenarios include offloading traffic off legacy networks for capacity improvement, bridging connectivity gaps, or deploying ad hoc networks in challenging environments for coverage enhancement.

==> 1c-mobile-entities-old.tex <==
\section{Mobile entities}
\label{sec:entities}

A number of mobile entities have been considered in the literature to carry out the role of data carriers. In this section, we first give a generic model for the alternative communication channel that results from the mobile entity movements. Second, we classify these entities according to the predictability of their mobility. 

\input{../../classification-tree.tex}

\input{table_classification_challenges_r2.tex}

\subsection{Mobile entity model}

A mobile entity can refer to humans, animals or vehicles equipped with storage devices, such as magnetic disks or other non-volatile solid-state storage devices. They are further equipped with communication capabilities such as wireless interfaces to support data exchange with other entities. The entities may also host the application responsible for producing or consuming the data while they move. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/entitiesv2D.pdf}
    \caption{Classification of entities mobile by nature or by design as a function of the degree of predictability of their mobility.}
    \label{fig:mobile-entities}
\end{figure}


\smallskip\noindent\textbf{Virtual links.} The movement of the entities so equipped enable data transfers from anywhere on the trajectories of the entities. As a result, the entity movements create virtual links analogous to physical links between routers. Contrary to physical links \del{were}\add{where} bits are propagated \del{in}\add{on} the wire, the virtual links result from the movements of the entities carrying data. Common network link metrics apply to the virtual links, which can be characterized in terms of bit error rate, throughput, and propagation delay. As it is the case in networks, the virtual link performance depends on the underlying entity that carries the data. As depicted in Figure~\ref{fig:mobile-entities}, the entities are capable of moving either by design (\eg mechanical vehicles powered by combustion or electric engines) or by nature (\eg living beings such as animals or humans carrying devices). 


\smallskip\noindent\textbf{Virtual routers.} In conventional networks, the purpose of physical links is to connect routers and hosts together to enable end-to-end data transfers. In the case of indirect data delivery, successive entities carry the data, which follows a sequence of entity movements connected together when passing the data. The data passing can either happen between two entities in a synchronous manner or asynchronously through intermediate relay nodes such as ferries~\cite{zhao2004message} or throwboxes~\cite{zhao2006capacity} bridging entities. Synchronous or asynchronous data passing then behaves as a virtual router between virtual links. The equivalent of output links in virtual router are the different entities available to pass the data, depending on the destination of the data. The data passing choice is therefore limited to whether the entity with the data should keep it, pass it, or replicate it to another entity.

\subsection{Entity-enabled data transfer scenarios}

Selecting the entities is crucial for the performance of the resulting data transfers. The selection mainly depends on the target environment where entities may be already living or operating. 

\smallskip\noindent\textbf{Sparse environments.} In sparse environments where few entities are available, one can exploit their movements to create a single virtual link connecting the endpoints of the data transfer, as the entities carry data directly from the source to the destination of the transfer. They can be grape pickers used to collect sensor data in vineyards~\cite{burrell2004vineyard} or buses connecting remote areas by transporting data as part of their regular service~\cite{pentland2004daknet}. Such entities are referred to as \textit{data mules} and have more or less predictable movements, depending on the entity. Mobility predictability increases the level of knowledge regarding the trajectory taken by the entities and the benefit of instrumenting their mobility.

\smallskip\noindent\textbf{Dense environments.} As more entities become available in dense environments, data transfers can involve multiple virtual routers connected by the entity movements. The virtual links result from the movements of each mobile entity carrying data and the virtual routers correspond to the data passing between two entities. This is the case of underwater ad hoc networks where whales equipped with sensors contribute to the collection and the transmission of sensed data~\cite{small2003shared}. In the savanna, zebras can act as data carriers but also as producers of environmental data that tracks their wildlife~\cite{juang2002energy}. 

\smallskip\noindent\textbf{Intermediate relay nodes.} The quest for predictability has also motivated the deployment of dedicated intermediate static or mobile relay nodes to increase the performance of data transfers. On the one hand, \textit{throwboxes} are static nodes that behave as virtual routers by enabling entities to buffer the data they carry before passing it to another entity. Virtual links are then the result of the entity movements between data passing\del{s} with other entities or throwboxes. Throwboxes are typically deployed in urban environments~\cite{zhao2006capacity} or in remote areas at rural kiosk locations~\cite{guo2007very}. On the other hand, \textit{data ferries} are controllable mobile nodes such as robots that act as virtual links by carrying data. They help bridging the connectivity between transfer endpoints or between entities. Virtual routers result from data passing\del{s} between the ferries and entities either picking up or dropping off data. The ferries can be autonomous underwater vehicles collecting data from underwater sensors~\cite{partan2007survey} or dedicated vehicles in challenged environments carrying data between strategic locations (\eg battlefields or disaster scenarios)~\cite{zhao2004message}.

\smallskip\noindent\textbf{\del{Paid}\add{Paying} parcel delivery services.} Finally, paid parcel delivery services create a virtual link connecting the transfer endpoints~\cite{wang2004turning}. Nevertheless, while the source and destination of the transfers are chosen, the calculation of the routes followed by the parcel are determined by the delivery services and cannot be controlled. Given the bandwidth resulting from the number of devices that can be shipped and the geographical coverage, paid parcel delivery service have been considered for assisting conventional data networks by offloading large amounts of data.  

Figure~\ref{fig:classification-survey} summarizes the classification according to the data delivery approaches we present in the survey. To complement this figure, \del{Table~\ref{tab:classification-challenges} summarizes all the data delivery approaches along with their recurring challenges and tradeoffs. Finally,} Table~\ref{tab:classification} summarizes the solutions and variations of the different data delivery approaches. Both tables are divided into the direct and indirect delivery approaches.




==> 6a-classification.tex <==
\section{Classification}
\label{sec:classification}

In this section, we provide a comprehensive classification of the existing solutions. We represent the structure of the classification in Figure~\ref{fig:classification-survey}. At a high level, we classify the techniques into the following two types:
\begin{itemize}
  \item Direct data delivery with a single entity used to deliver the data.
  \item Indirect data delivery with the composition of the trajectories of multiple entities to deliver the data.
\end{itemize}

We summarize the classification of the works in Table~\ref{tab:classification} according to the direct and indirect data delivery. We further classify the works according to other dimensions we detail in the following for each type of data delivery.

\smallskip\noindent\textbf{Direct data delivery.} Some works propose the use of a single entity to carry the data from its source all the way to the final destination. This results in a \textit{direct data delivery}, which we present in Section~\ref{sec:direct-delivery}. Using the existing mobility of entities provides a simple way to transfer data. However, the knowledge of their mobility is variable, which can results in data transfers with poor guarantees in terms of delivery delay data losses. To increase the guarantee of the data transfers, some works proposed to leverage entities with controlled mobility. Controlling their visits to static nodes (\eg sensors) allows better guarantee on the data transfers. Finally, instead of controlling oneself the entities' movements, one can contract services from third-parties to deliver the data. 

However, relying on a single entity is limiting regarding the expected benefits of using their mobility to transport data (\eg capacity or coverage). The idea of composing the trajectories of multiple entities was thus introduced to increase the capacity and the scale of the data transfers.

\smallskip\noindent\textbf{Indirect data delivery.} According to this idea, the data follows a path consisting of multiple segments of trajectories, each followed by different mobile entities. This results in an \textit{indirect data delivery}, which we present in Section~\ref{sec:indirect-delivery}. Data is passed from one entity to another as a result of the forwarding when entities are in direct contact.

In the case of indirect data delivery, the works we choose to present in this survey propose different strategies for composing the trajectories of mobile entities. Those strategies differ depending on the two following criteria:

\begin{itemize}
  
    \item The \textit{time} when composition should occur. The data can be passed either \textit{synchronously} at the time two entities meet or buffered before passed \textit{asynchronously} to subsequent entities.  
    \item The \textit{location} where composition is performed. The location can be either \textit{pre-positioned} or \textit{floating}. In the pre-positioned case, the data is passed if the entities are in contact at specific locations. In the floating case, composition results of contacts between entities regardless where they are in contact.

\end{itemize}

These two criteria correspond to two orthogonal dimensions, which create four combinations, as shown in Table~\ref{tab:classification}. The indirect data delivery strategies proposed in the literature result of the combination of one of each instance of both criteria. 

\input{table_classification.tex}

==> 6b-environment.tex <==
\section{Application scenarios}
The work covered in this survey have been conducted with application scenarios in mind which can be classified according to different criteria. A first criterion refers to the relation between the carrying entities and the communication endpoints responsible for sending or receiving the data. In scenarios involving a conventional data network, endpoints belong to this network and as so inherit the properties of the other nodes in the data network. Other scenarios are standalone as they make no assumptions regarding any existing communication network dedicated to data transmission. In both scenarios, entities are not necessary computer devices as they can refer to any entity capable to move as long as equipped with storage capabilities and communication interfaces. In the next section, we will review the different types of entities proposed as data carriers in the literature.       

In the first scenarios, mobile entities equipped with storage supplement a conventional data network to overcome limitations such as connectivity or capacity. In scenarios focusing on extending network connectivity, the objectives is to cover areas where the cost of deploying a communication infrastructure is prohibitively high due to restrictions deriving from the type of environment or the lack of financial means. Typical environments include underwater regions, opponents’ battlespace in armed conflicts, or rural areas in developing regions. Endpoints act as gateways where data is exchanged with the data network using mostly wireless technologies. 

Scenarios focusing on extending the network capacity refer to the emerging paradigm of offloading. Part or all the data of a transfer is transloaded from the data network to another mode of transportation typically involving mechanical vehicles such as cars, airplanes or trains. Those mobile entities are equipped with storage devices to act as data carriers and differ from the network endpoints. As so those scenario are similar to intermodal transportation systems involving different modes of transportation for freight or passengers. Their objective is to provide a virtual link resulting of their movements between the endpoints. Such link may be characterized by the aggregated capacity resulting from the entities’ combined storage. The flow of mobile entities act as an ancillary transmission medium that can help cope with the resource scarcity of legacy computer networks. 

When using mechanical vehicles such cars or trucks, the mobile entities may either be part of a fleet operated by a parcel delivery company. The trajectory of the trucks may be tracked using the online services provided by the delivery company. If a pickup and delivery can be arranged, the trajectory itself is controlled by the delivery company. A dray system may be required to bridge the network entry and exit points The service may be provided to a content provider with bulk data to migrate. Network operators can also benefit of this ancillary medium to offload background traffic from their network. 

Vehicles may also be used By stowing away data onto the entities’ embedded storage,  is expected to bring various benefits depending if the objective is to replace or supplement an existing infrastructure or 

In scenarios not relying on the existence a conventional network for data transmission, nodes may act as endpoints or forwarder. Nodes also host the applications generating or consuming the data carried by the mobile nodes. Such data may result a set of sensors. the gathering of data sensed 
